A Perspective on Symbolic Machine Learning in Physical Sciences

Machine learning is rapidly making its pathway across all of the natural sciences, including physical sciences. The rate at which ML is impacting non-scientific disciplines is incomparable to that in the physical sciences. This is partly due to the uninterpretable nature of deep neural networks. Symbolic machine learning stands as an equal and complementary partner to numerical machine learning in speeding up scientific discovery in physics. This perspective discusses the main differences between the ML and scientific approaches. It stresses the need to develop and apply symbolic machine learning to physics problems equally, in parallel to numerical machine learning, because of the dual nature of physics research.

==> taxonomy.tex <==
\setbox\mybox=\hbox{%
  \begin{forest}
    for tree={circle,draw}
    [a[b][c]]
  \end{forest}%
}
\tikzset{
    my node/.style={
        align=center,
        draw=black,
        inner color=white,%gray!5,
        outer color=white,%gray!10,
        thick,
        minimum width=0.9cm,
        rounded corners=3,
        text width=2.35cm,
    %    text height=4ex,
    %    text depth=1ex,
        font=\sffamily,
%        rectangle,
%       drop shadow,
    }
}
\begin{figure*}[t]
\centering 
\resizebox{0.5\textwidth}{!}{
\begin{forest}
    for tree={%
        my node,
        % where level=0{my node=blue,text width=6em}{},
        % where level=1{my node=purple,text width=5em}{},
        where level=4{text width=2em}{},
        l sep+=5pt,
        grow'=east,
        edge={gray, thick},
        parent anchor=east,
        child anchor=west,
        if n children=0{tier=last}{},
        edge path={
            \noexpand\path [draw, \forestoption{edge}] (!u.parent anchor) -- +(10pt,0) |- (.child anchor)\forestoption{edge label};
        },
        if={isodd(n_children())}{
            for children={
                if={equal(n,(n_children("!u")+1)/2)}{calign with current}{}
            }
        }{}
    }
    [ML in physical sciences
    [Numerical ML
    
    ]
    [Symbolic ML
    [Theoretical Calculations
    ]
    [Scientific Discovery
    ]
    ]
    ]
  \end{forest}
  }
  \\[5pt]
  \caption{}%Taxonomy based on the type of symbolic regression methods. $\phi$ denotes a neural network function, $W$ denotes the set of learnable parameters in NN. $\mathbf{x}$ denotes the input data, $\mathbf{z}$ denotes a reduced representation of $\mathbf{x}$, and $\mathbf{x}^{\prime}$ denotes a new representation of $\mathbf{x}$, e.g., by defining new features based on the original ones. $\mathcal{T}$ represents the final population of selected expression trees in genetic programming.}
  \label{fig:srtaxonomy}
\end{figure*}


% \tikzset{
%     my node/.style={
%         align=center,
%         draw=black,
%         inner color=white,%gray!5,
%         outer color=white,%gray!10,
%         thick,
%         minimum width=0.9cm,
%         rounded corners=3,
%     %    text width=2.7cm,
%     %    text height=4ex,
%     %    text depth=1ex,
%         font=\sffamily,
% %        rectangle,
% %       drop shadow,
%     }
% }

% \begin{figure}[h]
%     \centering
%     \begin{forest}
%     for tree={%
%         my node,
%         l sep+=5pt,
%         grow'=east,
%         edge={gray, thick},
%         child anchor=north,
%         parent anchor=south,
%         grow=south,
%         align=center,
%         edge path={
%         \noexpand\path[line width=1pt, \forestoption{edge}]
%         (!u.parent anchor)  |- ([yshift=4pt].child anchor) -- (.child anchor) \forestoption{edge label};
%         },
%         % parent anchor=east,
%         % child anchor=west,
%         if n children=0{tier=last}{},
%         % edge path={
%         %     \noexpand\path [draw, \forestoption{edge}] (!u.parent anchor) -- +(10pt,0) |- (.child anchor)\forestoption{edge label};
%         % },
%         if={isodd(n_children())}{
%             for children={
%                 if={equal(n,(n_children("!u")+1)/2)}{calign with current}{}
%             }
%         }{}
%     }
%     [SR Benchmark
%     [Ground-truth problems[Physics equations][Mathematics equations]]
%     [Real-world problems[Observations][Measurements]]
%     ]
%     \end{forest}
%     %\includegraphics[width=.9\linewidth]{plots/Taxonomy_data.png}
%     \caption{Taxonomy based on the type of SR benchmark problems.}
%     \label{fig:taxonomy_data}
% \end{figure}
